Solving Hierarchical Information-Sharing Dec-POMDPs: An Extensive-Form Game Approach

A recent theory shows that a multi-player decentralized partially observable Markov decision process can be transformed into an equivalent single-player game, enabling the application of \citeauthor{bellman}'s principle of optimality to solve the single-player game by breaking it down into single-stage subgames. However, this approach entangles the decision variables of all players at each single-stage subgame, resulting in backups with a double-exponential complexity. This paper demonstrates how to disentangle these decision variables while maintaining optimality under hierarchical information sharing, a prominent management style in our society. To achieve this, we apply the principle of optimality to solve any single-stage subgame by breaking it down further into smaller subgames, enabling us to make single-player decisions at a time. Our approach reveals that extensive-form games always exist with solutions to a single-stage subgame, significantly reducing time complexity. Our experimental results show that the algorithms leveraging these findings can scale up to much larger multi-player games without compromising optimality.

==> log_backup_time.tex <==


recycling hPBVI [3] [0.04202033333333333]
recycling hPBVI [3, 6] [0.04202033333333333, 7.175175666666665]
recycling hPBVI [3, 6, 8] [0.04202033333333333, 7.175175666666665, 94.57884233333334]
recycling PBVI [3] [135.84343199999998]
recycling PBVI [3, 6] [135.84343199999998, 10.0]
recycling PBVI [3, 6, 8] [135.84343199999998, 10.0, 10.0]
recycling PBVI_MILP [3] [15.928217333333334]
recycling PBVI_MILP [3, 6] [15.928217333333334, 10.0]
recycling PBVI_MILP [3, 6, 8] [15.928217333333334, 10.0, 10.0]
=== save figure: ./figures/backup_time/recycling_h30


==> tableNew1.tex <==
\begin{tabular}{l|cc|cc|cc||cc|cc}
\toprule
  %Algorithm &  $t$ & ($num it$) & $\bar{\underline{\upsilon}}_0(s_0)$ & $\underline{\underline{\upsilon}}_0(s_0)$ &  $gap(s_0)$ & $size(\bar{\underline{\upsilon}})$ & $size(\underline{\underline{\upsilon}})$size(\bar{\underline{\upsilon}})$ & $size(\underline{\underline{\upsilon}})$\\
\multicolumn{1}{c|}{} & \multicolumn{2}{c|}{PBVI$_3$} & \multicolumn{2}{c|}{PBVI$_2$} & \multicolumn{2}{c||}{PBVI$_1$} & \multicolumn{2}{c|}{A2C} & \multicolumn{2}{c}{IQL}\\
 & \multicolumn{1}{c}{\# B}& \multicolumn{1}{c|}{$\underline{\upsilon}_0(b_0)$} & \multicolumn{1}{c}{\# B}& \multicolumn{1}{c|}{$\underline{\upsilon}_0(b_0)$} & \multicolumn{1}{c}{\# B}& \multicolumn{1}{c||}{$\underline{\upsilon}_0(b_0)$}& \multicolumn{1}{c}{\# it}& \multicolumn{1}{c|}{$\underline{\upsilon}_0(b_0)$} & \multicolumn{1}{c}{\# it}& \multicolumn{1}{c}{$\underline{\upsilon}_0(b_0)$}\\
\multicolumn{1}{c|}{$n$}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{} & \multicolumn{1}{c}{}& \multicolumn{1}{c|}{} & \multicolumn{1}{c}{}& \multicolumn{1}{c||}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{} & \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\midrule 
%
%
%pb: Problem: Tiger horizon 30 agents 3 : {'Problem: Tiger horizon 30 agents 3,hPBVI': [262.500031, 12], 'Problem: Tiger horizon 30 agents 3,PBVI': [262.500031, 3], 'Problem: Tiger horizon 30 agents 3,PBVI_MILP': [262.500031, 4], 'Problem: Tiger horizon 30 agents 3,A2C': [190.37792695326542, 89017852], 'Problem: Tiger horizon 30 agents 3,IQL': [31.718876, 76365856]}
%pb: Problem: Tiger horizon 30 agents 6 : {'Problem: Tiger horizon 30 agents 6,hPBVI': [649.999939, 14], 'Problem: Tiger horizon 30 agents 6,A2C': [496.44657915019474, 31507264], 'Problem: Tiger horizon 30 agents 6,IQL': [-89.18661176119136, 43909298]}
%pb: Problem: Tiger horizon 30 agents 8 : {'Problem: Tiger horizon 30 agents 8,hPBVI': [1012.5, 2], 'Problem: Tiger horizon 30 agents 8,A2C': [738.2256091483546, 14627730], 'Problem: Tiger horizon 30 agents 8,IQL': [-16.956947, 19331381]}
%
%
%Problem: Tiger horizon 30 agents 2': {'Problem: Tiger horizon 30 agents 2,hPBVI': [112.5, 12], 'Problem: Tiger horizon 30 agents 2,PBVI': [112.5, 10], 'Problem: Tiger horizon 30 agents 2,PBVI_MILP': [112.5, 8], 'Problem: Tiger horizon 30 agents 2,A2C': [94.04658110125422, 128732864], 'Problem: Tiger horizon 30 agents 2,IQL': [20.55107633333333, 98179915]}, 
%'Problem: Tiger horizon 30 agents 4': {'Problem: Tiger horizon 30 agents 4,hPBVI': [393.749969, 13], 'Problem: Tiger horizon 30 agents 4,A2C': [218.49203716483862, 60622607], 'Problem: Tiger horizon 30 agents 4,IQL': [-74.07377633333334, 52289398]},
\multicolumn{11}{c}{\it $\mathtt{tiger}$ $|X|=2,~|U^i|=3,~|Z^i|=2$}\\
\midrule
  %\rowcolor[gray]{.95}[.5\tabcolsep] 
   %HSVI$_1(1)$ & {0.004} & (10) & $9.2901$ & $9.2901$ & $0.0$ & 20 & 20 &\\
   %\multirow{2}{*}{$\ell=30$}
   %&
   $2$ & $\pgfmathprintnumber{0.02}$s & $\boldsymbol{112.5}$ & $\pgfmathprintnumber{0.20}$s & $\boldsymbol{112.5}$ & $\pgfmathprintnumber{0.05}$s &  $\boldsymbol{112.5}$ &$\pgfmathprintnumber{128732864}$&$94.05$&$\pgfmathprintnumber{98179915}$&$20.55$\\
   $3$ & $\pgfmathprintnumber{0.07}$s & $\boldsymbol{262.5}$ & $\pgfmathprintnumber{16.03}$s & $\boldsymbol{262.5}$ & $\pgfmathprintnumber{14.25}$s &  $\boldsymbol{262.5}$ &$\pgfmathprintnumber{89017852}$&$190.38$&$\pgfmathprintnumber{76365856}$&$31.72$\\
   $4$ & $\pgfmathprintnumber{0.23}$s & $\boldsymbol{393.75}$ & - & - & - &  - &$\pgfmathprintnumber{60622607}$&$218.49$&$\pgfmathprintnumber{52289398}$&$-74.07$\\
   %&
   $6$ & $\pgfmathprintnumber{8.12}$s & $\boldsymbol{650}$ & - & - & - & - &$\pgfmathprintnumber{31507264}$&$496.45$&$\pgfmathprintnumber{43909298}$&$-89.18$\\
   %&
   $8$ & $\pgfmathprintnumber{864.03}$s & $\boldsymbol{1012.5}$ & - & - & - & - &$\pgfmathprintnumber{14627730}$&$738.22$&$\pgfmathprintnumber{9331381}$&$-16.95$\\
\midrule 
\multicolumn{11}{c}{\it $\mathtt{Recycling}$ $|X|=2^{N},~|U^i|=3,~|Z^i|=2$}\\
\midrule
%
%pb: Problem: Recycling robots horizon 30 agents 3 : {'Problem: Recycling robots horizon 30 agents 3,hPBVI': [140.357437, 12], 'Problem: Recycling robots horizon 30 agents 3,PBVI': [140.357437, 3], 'Problem: Recycling robots horizon 30 agents 3,PBVI_MILP': [140.357437, 3], 'Problem: Recycling robots horizon 30 agents 3,A2C': [140.38515619246243, 91626669], 'Problem: Recycling robots horizon 30 agents 3,IQL': [140.357437, 70809846]}
%pb: Problem: Recycling robots horizon 30 agents 6 : {'Problem: Recycling robots horizon 30 agents 6,hPBVI': [280.714874, 7], 'Problem: Recycling robots horizon 30 agents 6,A2C': [256.3923593794625, 25269178], 'Problem: Recycling robots horizon 30 agents 6,IQL': [279.8855419691603, 46065122]}
%pb: Problem: Recycling robots horizon 30 agents 8 : {'Problem: Recycling robots horizon 30 agents 8,hPBVI': [345.8456890914073, 4], 'Problem: Recycling robots horizon 30 agents 8,A2C': [331.0046363773158, 21036122]}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% new version of recycling %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%pb: Problem: Recycling robots horizon 30 agents 3 : {'Problem: Recycling robots horizon 30 agents 3,hPBVI': [229.5, 12], 'Problem: Recycling robots horizon 30 agents 3,PBVI': [223.5, 3], 'Problem: Recycling robots horizon 30 agents 3,PBVI_MILP': [229.5, 5], 'Problem: Recycling robots horizon 30 agents 3,A2C': [139.11769700082635, 45395220], 'Problem: Recycling robots horizon 30 agents 3,IQL': [128.661942, 69111743]}
%pb: Problem: Recycling robots horizon 30 agents 6 : {'Problem: Recycling robots horizon 30 agents 6,hPBVI': [459.0, 8], 'Problem: Recycling robots horizon 30 agents 6,A2C': [-50.715307673124585, 18260338], 'Problem: Recycling robots horizon 30 agents 6,IQL': [204.2471393161924, 49289524]}
%
%pb: Problem: Recycling robots horizon 30 agents 8 : {'Problem: Recycling robots horizon 30 agents 8,hPBVI': [381.979431, 4], 'Problem: Recycling robots horizon 30 agents 8,A2C': [-110.10925285784755, 20752135], 'Problem: Recycling robots horizon 30 agents 8,IQL': [251.730835, 25636665]}
%
%pb: Problem: Recycling robots horizon 30 agents 2 : {'Problem: Recycling robots horizon 30 agents 2,hPBVI': [93.727783, 13], 'Problem: Recycling robots horizon 30 agents 2,PBVI': [93.727783, 10], 'Problem: Recycling robots horizon 30 agents 2,PBVI_MILP': [93.727783, 7], 'Problem: Recycling robots horizon 30 agents 2,A2C': [93.41848, 80807057], 'Problem: Recycling robots horizon 30 agents 2,IQL': [93.2543383163044, 95970308]}
%pb: Problem: Recycling robots horizon 30 agents 4 : {'Problem: Recycling robots horizon 30 agents 4,hPBVI': [306.0, 10], 'Problem: Recycling robots horizon 30 agents 4,PBVI_MILP': [258.942505, 2], 'Problem: Recycling robots horizon 30 agents 4,A2C': [166.67507427156713, 61522235], 'Problem: Recycling robots horizon 30 agents 4,IQL': [153.1799706222563, 51334298]}
   %\multirow{2}{*}{$\ell=30$}
   %&
   $2$ & $\pgfmathprintnumber{0.02}$s & $\boldsymbol{93.73}$ & $\pgfmathprintnumber{0.61}$s & $\boldsymbol{93.73}$ & $\pgfmathprintnumber{0.04}$s &  $\boldsymbol{93.73}$ &$\pgfmathprintnumber{131389573}$&$93.37$&$\pgfmathprintnumber{89902007}$&$93.22$\\
   $3$ & $\pgfmathprintnumber{0.042}$s & $\boldsymbol{229.5}$ & $\pgfmathprintnumber{15.93}$s & $\boldsymbol{229.5}$ & $\pgfmathprintnumber{135.84}$s & $223.5$ &$\pgfmathprintnumber{45395220}$&$139.12$&$\pgfmathprintnumber{69111743}$&$128.66$\\
   %&
   $4$ & $\pgfmathprintnumber{0.13}$s & $\boldsymbol{306.0}$ & $\pgfmathprintnumber{1148.82}$s & $258.94$ & - &  - &$\pgfmathprintnumber{61522235}$&$166.68$&$\pgfmathprintnumber{51334298}$&$154.18$\\
   $6$ & $\pgfmathprintnumber{7.18}$s & $\boldsymbol{459.0}$ & - & - & - & - &$\pgfmathprintnumber{18260338}$&$-50.71$&$\pgfmathprintnumber{49289524}$&$204.25$\\
   %&
   $8$ & $\pgfmathprintnumber{94.58}$s & $\boldsymbol{381.898}$ & - & - & - & - &$\pgfmathprintnumber{20752135}$&$-110.11$&$\pgfmathprintnumber{25636665}$&$251.73$\\
\midrule 
\multicolumn{11}{c}{\it $\mathtt{mabc}$ $|X|=2^{N},~|U^i|=2,~|Z^i|=2$}\\
\midrule
%
%pb: Problem: Broadcast horizon 30 agents 3 : {'Problem: Broadcast horizon 30 agents 3,hPBVI': [23.235695, 12], 'Problem: Broadcast horizon 30 agents 3,PBVI': [23.235695, 7], 'Problem: Broadcast horizon 30 agents 3,PBVI_MILP': [23.235695, 7], 'Problem: Broadcast horizon 30 agents 3,A2C': [23.272116387631964, 95685831], 'Problem: Broadcast horizon 30 agents 3,IQL': [23.235695, 83939464]}
%pb: Problem: Broadcast horizon 30 agents 7 : {'Problem: Broadcast horizon 30 agents 7,hPBVI': [27.247368, 8], 'Problem: Broadcast horizon 30 agents 7,A2C': [16.720427104148147, 27903848]}
%pb: Problem: Broadcast horizon 30 agents 10 : {'Problem: Broadcast horizon 30 agents 10,hPBVI': [27.751180922598326, 4], 'Problem: Broadcast horizon 30 agents 10,A2C': [12.249208783421421, 18422015], 'Problem: Broadcast horizon 30 agents 10,IQL': [24.843082, 20793345]}
%
%pb: Problem: Broadcast horizon 30 agents 2 : {'Problem: Broadcast horizon 30 agents 2,hPBVI': [27.421844000000004, 14], 'Problem: Broadcast horizon 30 agents 2,PBVI': [27.421844000000004, 14], 'Problem: Broadcast horizon 30 agents 2,PBVI_MILP': [27.404754333333333, 9], 'Problem: Broadcast horizon 30 agents 2,A2C': [27.18446493882044, 132264112], 'Problem: Broadcast horizon 30 agents 2,IQL': [27.199992999999996, 113337638]}
%
%pb: Problem: Broadcast horizon 30 agents 4 : {'Problem: Broadcast horizon 30 agents 4,hPBVI': [24.935461, 11], 'Problem: Broadcast horizon 30 agents 4,PBVI_MILP': [24.935461, 3], 'Problem: Broadcast horizon 30 agents 4,A2C': [24.360780057649862, 65719650], 'Problem: Broadcast horizon 30 agents 4,IQL': [24.935461, 61922214]}
%
   %\multirow{3}{*}{$\ell=30$}
   %&
   $2$ & $\pgfmathprintnumber{0.05}$s & $\boldsymbol{27.42}$ & $\pgfmathprintnumber{0.15}$s & $27.40$ & $\pgfmathprintnumber{0.04}$s &  $\boldsymbol{27.42}$ &$\pgfmathprintnumber{132264112}$&$27.18$&$\pgfmathprintnumber{113337638}$&$27.2$\\
   $3$ & $\pgfmathprintnumber{0.03}$s & $23.24$ & $\pgfmathprintnumber{1.21}$s & $23.24$ & $\pgfmathprintnumber{0.65}$s & $23.24$&$\pgfmathprintnumber{95685831}$&$\boldsymbol{23.27}$&$\pgfmathprintnumber{83939464}$&$23.24$\\
   %&
      $4$ & $\pgfmathprintnumber{0.07}$s & $\boldsymbol{24.94}$ & $\pgfmathprintnumber{223.26}$s & $24.94$ & - &  - &$\pgfmathprintnumber{65719650}$&$\boldsymbol{24.36}$&$\pgfmathprintnumber{61922214}$&$\boldsymbol{24.94}$\\
   $7$ & $\pgfmathprintnumber{1.66}$s & $\boldsymbol{27.25}$ & - & - & - & - &$\pgfmathprintnumber{27903848}$&$16.72$&?&?\\
   %&
   $10$ & $\pgfmathprintnumber{139.82}$s & $\boldsymbol{27.75}$ & - & - & - & - &$\pgfmathprintnumber{18422015}$&$12.25$&$\pgfmathprintnumber{20793345}$&$24.84$\\
\midrule 
\multicolumn{11}{c}{\it $\mathtt{Grid3x3}$ $|X|=9^{N},~|U^i|=5,~|Z^i|=9,~|O|\approx 1.3 \cdot  10^{1019}$}\\
\midrule
%
%pb: Problem: Meeting in a 3x3 grid horizon 30 agents 2 : {'Problem: Meeting in a 3x3 grid horizon 30 agents 2,hPBVI': [24.438486950392033, 10], 'Problem: Meeting in a 3x3 grid horizon 30 agents 2,PBVI_MILP': [24.327883, 2], 'Problem: Meeting in a 3x3 grid horizon 30 agents 2,A2C': [22.92776997925022, 107097171], 'Problem: Meeting in a 3x3 grid horizon 30 agents 2,IQL': [24.348410236603087, 98395369]}
%pb: Problem: Meeting in a 3x3 grid horizon 30 agents 3 : {'Problem: Meeting in a 3x3 grid horizon 30 agents 3,hPBVI': [28.162989, 6], 'Problem: Meeting in a 3x3 grid horizon 30 agents 3,A2C': [28.196760490004195, 36028833], 'Problem: Meeting in a 3x3 grid horizon 30 agents 3,IQL': [28.153393231038844, 26190075]}
%
   %\multirow{3}{*}{$\ell=30$}
   %&
   $2$ & $\pgfmathprintnumber{0.61}$s & $\boldsymbol{24.44}$ & $\pgfmathprintnumber{1329.33}$s&$24.33$  & - & -&$\pgfmathprintnumber{107097171}$ &$22.93$&$\pgfmathprintnumber{98395369}$&$24.35$\\
   %&
   $3$ & $\pgfmathprintnumber{65.43}$s & $28.16$ & - & - & - & - &$\pgfmathprintnumber{36028833}$&$\boldsymbol{28.20}$&$\pgfmathprintnumber{26190075}$&$28.16$\\
\midrule 
\multicolumn{11}{c}{\it $\mathtt{Mars}$ $|X|=256,~|U^i|=6,~|Z^i|=8$}\\
\midrule
%
%pb: Problem: Mars rover horizon 30 agents 2 : {'Problem: Mars rover horizon 30 agents 2,hPBVI': [84.32575573164348, 10], 'Problem: Mars rover horizon 30 agents 2,PBVI_MILP': [76.15282451302859, 3], 'Problem: Mars rover horizon 30 agents 2,A2C': [43.19665141214977, 105183330], 'Problem: Mars rover horizon 30 agents 2,IQL': [52.86059521712359, 90474497]}
%
   %\multirow{3}{*}{$\ell=30$}
   %&
   $2$ & $\pgfmathprintnumber{0.28}$s & $\boldsymbol{84.33}$ & $\pgfmathprintnumber{248.61}$s & $76.15$ & - & - &$\pgfmathprintnumber{105183330}$&$43.20$&$\pgfmathprintnumber{90474497}$&$52.86$\\
\midrule 
\multicolumn{11}{c}{\it $\mathtt{BoxPushing}$ $|X|=100,~|U^i|=4,~|Z^i|=5$}\\
\midrule
%
%pb: Problem: Box-pushing horizon 30 agents 2 : {'Problem: Box-pushing horizon 30 agents 2,hPBVI': [675.459656, 10], 'Problem: Box-pushing horizon 30 agents 2,PBVI_MILP': [576.295837, 4], 'Problem: Box-pushing horizon 30 agents 2,A2C': [180.11265115843187, 121523549], 'Problem: Box-pushing horizon 30 agents 2,IQL': [614.5978819844688, 146378742]}
%
   %\multirow{3}{*}{$\ell=30$}
   %&
   $2$ & $\pgfmathprintnumber{0.66}$s & $\boldsymbol{675.46}$ & $\pgfmathprintnumber{24.58}$s & $576.30$ & - & - &$\pgfmathprintnumber{121523549}$&$180.11$&$\pgfmathprintnumber{146378742}$&$614.6$\\
\bottomrule
\end{tabular}

